Robust Trajectory Prediction against Adversarial Attacks

Trajectory prediction using deep neural networks (DNNs) is an essential component of autonomous driving (AD) systems. However, these methods are vulnerable to adversarial attacks, leading to serious consequences such as collisions. In this work, we identify two key ingredients to defend trajectory prediction models against adversarial attacks including (1) designing effective adversarial training methods and (2) adding domain-specific data augmentation to mitigate the performance degradation on clean data. We demonstrate that our method is able to improve the performance by 46% on adversarial data and at the cost of only 3% performance degradation on clean data, compared to the model trained with clean data. Additionally, compared to existing robust methods, our method can improve performance by 21% on adversarial examples and 9% on clean data. Our robust model is evaluated with a planner to study its downstream impacts. We demonstrate that our model can significantly reduce the severe accident rates (e.g., collisions and off-road driving).

==> method.tex <==


\section{Challenges}
\label{sec:challenges}
As stated above, applying adversarial training to trajectory prediction problems present three critical challenges.
\textbf{(i). Gradient obfuscation due to model stochasticity.} Since trajectory prediction is inherently uncertain and there is no single correct answer, probabilistic generative models are usually used to cope with the stochastic nature of the trajectory prediction task. Such stochasticity will obfuscate the gradients that are used to generate effective adversarial examples in the inner maximization process of adversarial training. It makes the whole adversarial training 
%in Eq.~\ref{eq:adv_train}
less effective. 
% A simple solution to handle such a stochasticity is to leverage Expectation Over Transformation (EoT) strategy. However, this method requires many samples to calculate the expectation, dramatically increasing the time complexity of adversarial training. 
\textbf{(ii). Unstable learning due to changing adversarial distribution.}
% In the adversarial training process, modeling $p_\theta(\mathbf{Y}|\mathbf{X}+\delta,\mathbf{Z})$  becomes substantially harder since $\mathbf{X}+\delta$ is a changing distribution (). 
% the modeling process becomes substantially harder since it needs to model the data distribution $p_\theta(\mathbf{Y}|\mathbf{X}+\delta,\mathbf{Z})$. 
During the adversarial training process,  $\mathbf{X}+\delta$ is a changing distribution since distribution of $\delta$ is calculated via an inner maximization process and thus not a deterministic distribution. 
Although $\delta$ is bounded by the adversarial set $\mathbb{S}_p^\epsilon$, the resulting latent condition variable $\mathbf{C}=f(\mathbf{X}+\delta)$ can be extremely large and noisy since there is the Lipschitz constant of neural network layers ($f$) is not bounded. 
% and  arbitrarily far from that of the unperturbed input
% , \textit{i.e.,}  $|f(\mathbf{X}+\delta) - f(\mathbf{X})|$ can be extremely large.
% so that  the conditional variable $\mathbf{C}=f(\mathbf{X}+\delta)$ could become arguably noisier. 
Since $\mathbf{C}=f(\mathbf{X}+\delta)$ is noisy and less informative, $p_\theta(\mathbf{Y}|\mathbf{X}+\delta,\mathbf{Z})$ tends to depend more upon $\mathbf{Z}$. It, thus, makes  modeling $p_\theta(\mathbf{Y}|\mathbf{X}+\delta,\mathbf{Z})$  becomes substantially harder
% The history trajectories are encoded into the conditional variable $\mathbf{C} = f(\mathbf{X})$  via a deep neural network. It can significantly enlarge the change from $\delta$~\cite{weng2018towards}.
% Hence, although the perturbation from $\delta$ is bounded by  $\mathbb{S}_p^\epsilon$, the resulting latent condition variable $\mathbf{C}=f(\mathbf{X}+\delta)$ can be arbitrarily far from that of the unperturbed input, \textit{i.e.,}  $|f(\mathbf{X}+\delta) - f(\mathbf{X})|$ can be large.
% As the conditional variable $\mathbf{C}=f(\mathbf{X}+\delta)$ becomes arguably noisier, the conditional distribution $p_\theta(\mathbf{Y}|\mathbf{X}+\delta,\mathbf{Z})$ tends to depend more upon $\mathbf{Z}$.
\danfei{This sentence is really hard to parse}This eventually makes the conditional generative model less depend on history trajectories and learn the adversarial robust space unstably. We will provide an empirical analysis in the later part of this section.
% During the adversarial training process,  $\mathbf{X}+\delta$ is a changing distribution since distribution of $\delta$ is calculated via inner maximization. The history trajectories are encoded into the conditional variable $\mathbf{C} = f(\mathbf{X})$  via a deep neural network. It can significantly enlarge the change from $\delta$~\cite{weng2018towards}.
% Hence, although the perturbation from $\delta$ is bounded by  $\mathbb{S}_p^\epsilon$, the resulting latent condition variable $\mathbf{C}=f(\mathbf{X}+\delta)$ can be arbitrarily far from that of the unperturbed input, \textit{i.e.,}  $|f(\mathbf{X}+\delta) - f(\mathbf{X})|$ can be large.
% As the conditional variable $\mathbf{C}=f(\mathbf{X}+\delta)$ becomes arguably noisier, the conditional distribution $p_\theta(\mathbf{Y}|\mathbf{X}+\delta,\mathbf{Z})$ tends to depend more upon $\mathbf{Z}$.
% This eventually makes the conditional generative model less depend on history trajectories and not learning the adversarial robust space stably.  
% In this case, it is hard for the model to learn the adversarial robust space stably.  
\textbf{(iii). Performance loss in benign situation.} Adversarial training often leads to performance degradation on clean data~\cite{defense:zhang2019theoretically}. However, trajectory prediction is a critical component for safety-critical AD systems and its the performance degradation can result in severe consequences (\textit{e.g.} collisions). Thus, it is important to balance the performance on the clean and adversarial data when designing adversarial training algorithms. \yulong{if degradation is shown in previous work, why is it a challenge? What is the unique point of our solution?}

% \begin{itemize}[leftmargin=8pt]\setlength\itemsep{-0em}
% \item Since trajectory prediction is inherently uncertain and there is no single correct answer, probabilistic generative models are usually used to cope with the stochastic nature of the trajectory prediction task. Such a stochasticity will obfuscate the gradients that are used to generate effective adversarial examples in the inner maximization process of adversarial training. It makes the whole adversarial training in Eq.~\ref{eq:adv_train} less effective.  A simple solution to handle such a stochasticity is to leverage Expectation Over Transformation (EoT) strategy. However, this method requires many samples to calculate the expectation, dramatically increasing the time complexity of adversarial training.   
% \item In the adversarial training process, the modeling process becomes substantially harder since it needs to model a data distribution $p_\theta(\mathbf{Y}|\mathbf{X}+\delta,\mathbf{Z})$. During the adversarial training process,  $\mathbf{X}+\delta$ is a changing distribution since distribution of $\delta$ is calculated via inner maximization. The history trajectories are encoded into the conditional variable $\mathbf{C} = f(\mathbf{X})$  via a deep neural network. It can significantly enlarge the change from $\delta$~\cite{weng2018towards}.
% On the other hand, although the perturbation from $\delta$ is bounded by the attack capability $\mathbb{S}_p^\epsilon$, the resulting latent condition variable $\mathbf{C}=f(\mathbf{X}+\delta)$ can be arbitrarily far from that of the unperturbed input, i.e.,  $|f(\mathbf{X}+\delta) - f(\mathbf{X})|$ can be large.
% As the conditional variable $\mathbf{C}=f(\mathbf{X}+\delta)$ becomes arguably noisier, the conditional distribution $p_\theta(\mathbf{Y}|\mathbf{X}+\delta,\mathbf{Z})$ tends to depend more upon $\mathbf{Z}$.
% On the other hand, this eventually will make the conditional generative model less depend on  history trajectories.
% In this case, it is hard for the model to learn the adversarial robust space stably.  
% \item Adversarial training often leads to performance degradation in clean cases~\cite{defense:zhang2019theoretically}. However, since trajectory prediction is a critical component for safety-critical AD systems, the performance degradation could result in severe consequences such as collision. Thus,  it is important to balance the performance on the clean and adversarial data when designing adversarial training algorithms. 

% \end{itemize}

\begin{figure}[t]
    \centering
    % \begin{minipage}{.06\textwidth}
    % \tiny
    %     \begin{tabular}{c}
    %          Cond.\\
    %          CVAE \\
    %          \\
    %          \\
    %          \\
    %           \\
    %           \\
    %           \\
    %           \\
    %           \\
    %     \end{tabular}
    % \end{minipage}
    \begin{minipage}{.24\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={0 5.2cm 0 0},clip]{figs/sample_all.png}
        \text{(a) Clean}
    \end{minipage}
    \begin{minipage}{.24\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={0 5.2cm 0 0},clip]{figs/sample_all_noise.png}
        \text{(b) Salt and pepper}
    \end{minipage}
    \begin{minipage}{.24\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={0 5.2cm 0 0},clip]{figs/sample_all_adv.png}
        \text{(c) Adv noise}
    \end{minipage}
    % \hfill
    \begin{minipage}{.24\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={0 0.6cm 0 1.0cm},clip]{figs/adv_ablation.png}
        \text{(d) Probability}
    \end{minipage}
    \caption{Visual examples for reconstruction with different methods. The first row shows the conditional variables and the rest of rows show the generated images based on the conditional variables. Each row of the generated images use the same random seed for sampling the latent prior value for CVAE. Here, we show the noise level of $p=0.1$ for salt and pepper noise and $\epsilon=0.1$ for the adversarial noises.}
    \vspace{-1em}
    \label{fig:cvae_analysis}
\end{figure}

% \textbf{Analysis on Noisy Conditional Variable}\label{sec:noisy}
\textbf{More Analysis on the Challenge \textbf{(ii)}.}\label{sec:noisy}
\danfei{Why is challenge 1 not part of it? Also there is 0 connection between the challenge and the analysis. There needs to be some sentences that connects the challenge and the necessity of analyzing the challenge. Why is analyzing MNIST a good proxy for explaining a problem in trajectory generation? The ``more analysis'' is very abrupt right now}
\chaowei{need to discuss}
To further demonstrate that it is hard to model  $p_\theta(\mathbf{Y}|\mathbf{X}+\delta,\mathbf{Z})$ with a changing data distribution of $X+\delta$, we conduct an analysis on a simplified task using MNIST dataset. Specifically, we divide each digit image into four quadrants, and take one quadrant as the input $X$ and the remaining quadrants as the output. We trained conditional generative models (CVAE) using clean ($X$) and noisy data ($X+\delta$). We selectively choose two kind of noises $\delta$: salt and pepper noise and adversarial noise. 
% We represent $X$ with different data including the clean data,  salt and pepper noise and  adversarial noise to CVAE model  $p_\theta(\mathbf{Y}|\mathbf{X}+\delta,\mathbf{Z})$, resulting in three models shown in Fig.~\ref{fig:cvae_analysis}.
As the results, three models trained with clean and noisy data are shown in Fig.~\ref{fig:cvae_analysis}.
The top-left region of each image in the first row is the conditional variables X. The rest of rows are the generated images with different $Z$. Each column in the same row uses the same $Z$. More experimental details are described in the appendix.\yulong{consistency check[appendix,Appendix]}
% Here, we consider two different noises: salt and pepper noise and adversarial noise. More experimental settings are show in the appendix.

We observe that model trained on clean data demonstrates the capability of generating multimodal images (the generated image highly depends on both $X$ and $Z$) while model trained with adversarial noise generates images independent of $X$ (i.e. each row generates images with the same digit). This result shows that the conditional generative model fails to learn from the $X$.
To provide a quantitative analysis, we train a simple classifier on MNIST achieving 99\% accuracy and show the average confidences of 10 generated samples being predicted as the label of $X$. In Fig.~\ref{fig:cvae_analysis} (d), we observe that the average score drops as the noise level increased. Therefore, we conclude that (1) the noises in the conditional data will degenerate the conditional generative model to a generative model solely dependent upon the sampled prior (i.e. CVAE to VAE), and (2) adversarial noises are more effective for such degeneration.



% \begin{figure}
%     \centering
%     \includegraphics[witdh=\textwidth]{figs/adv_ablation.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{table}[]
% \tiny
% \begin{minipage}{.3\textwidth}
%     \begin{tabular}{lccccc}
%         \toprule
%         Scale       & 0.00  & 0.01  & 0.03  & 0.05  & 0.1   \\\midrule
%         Probability & 0.607 & 0.506 & 0.420 & 0.378 & 0.183 \\\midrule
%         Std         & 0.276 & 0.240 & 0.164 & 0.167 & 0.090 \\\bottomrule
%     \end{tabular}
%     \caption{Training with different noise level for adversarial noise.}
% \end{minipage}
% \hfill
% \begin{minipage}{.65\textwidth}
%     \begin{tabular}{lcccccccccc}
%         \toprule
%         Scale       & 0.00  & 0.1   & 0.2   & 0.3   & 0.4   & 0.5   & 0.6   & 0.7   & 0.8   & 0.9   \\\midrule
%         Probability & 0.607 & 0.473 & 0.445 & 0.415 & 0.386 & 0.378 & 0.279 & 0.279 & 0.234 & 0.206 \\\midrule
%         Std         & 0.276 & 0.201 & 0.187 & 0.217 & 0.188 & 0.192 & 0.137 & 0.143 & 0.072 & 0.070 \\\bottomrule
%     \end{tabular}
%     \caption{Training with different noise level for salt and pepper noise.}
% \end{minipage}

% \end{table}

\section{\method{}: Robust Trajectory Prediction}
% Robust trajectory prediction aims to make models robust to adversarial attacks by formulating the adversarial training in the context of trajectory prediction task. In this section, we 
% % (1) introduce the preliminaries of trajectory prediction with conditional latent variable model, (2) present the challenges and overview of our proposed method, and (3) discuss the detailed methodology.
% describe the proposed \method{} for addressing the challenges mentioned in~\S\ref{sec:challenges}

% \subsection{Our Method}
We propose a new adversarial training framework to address the above challenges, named \method{}. Our method consists of three main components: 

\textbf{Component 1: Deterministic Attacks for Inner Maximization.}
In the inner maximization process, the goal is to generate effective adversarial examples to  exploit the {\em entire model} for training a robust model.
the na\"ive attack  mentioned in section~\ref{sec:pre} is a straightforward way to achieve this goal. However, this optimization involves a stochastic sampling process $Z^{(k)} \sim \mathcal{N}(p_\theta^\mu(Z|X),p_\theta^\sigma(Z|X))$. 
% To achieve this goal, the method should attack the {\em entire generative model} in an end-to-end manner. Therefore, an intuitive formulation of the attack is:
% % \begin{equation}
%     % \label{eq:sample_attack}
%     $\delta = \argmax_{\delta  \in \mathbb{S}} \{ \min_{k \in \{1, \cdots, K\}}\parallel p_\theta(\mathbf{Y|X + \delta}, \mathbf{Z}^{(k)})-\mathbf{Y}\parallel^2 \}$
% % \end{equation}
% % \begin{equation}
% %     \label{eq:sample_attack}
% %     \delta = \argmax_{\delta  \in \mathbb{S}} \min_{k \in \{1, \cdots, K\}}\parallel p_\theta(\mathbf{Y|X + \delta}, \mathbf{Z}^{(k)})-\mathbf{Y}\parallel^2
% % \end{equation}
% However, as shown in this equation,  this optimization involves a stochastic sampling process $Z^{(k)} \sim \mathcal{N}(p_\theta^\mu(Z|X),p_\theta^\sigma(Z|X))$.
Such the stochastic process will obfuscate the gradients for finding optimal adversarial perturbation $\delta$ to mislead the model, making the outer minimization (robust training) less effective. 
In order to bypass such stochasticity, we propose to generate the adversarial perturbation by using a {\em deterministic latent code} $\hat{Z}$. Specifically, we replace the sampling process $Z^{(k)} \sim \mathcal{N}(p_\theta^\mu(Z|X),p_\theta^\sigma(Z|X))$, with the maximum-likelihood sample (here, i.e $\hat{Z} = p_\theta^\mu(Z|X)$). The objective for generating the adversarial perturbation is thus:
\begin{equation}
\label{eq:adv_loss}
    \delta = \argmax_{\delta \in \mathbb{S}} \mathcal{L}_\text{adv} (\mathbf{X} + \delta, \mathbf{Y}) = \, \argmax_{\delta \in \mathbb{S}} \parallel p_\theta(\mathbf{Y}|\hat{Z},\mathbf{X+\delta}) -\mathbf{Y}\parallel^2 \text{where,} \hat{z} = p_\theta^\mu(Z|X+\delta) 
\end{equation}
We empirically show that gradients from this deterministic gradient path can effectively guide the generation of adversarial examples. We name our attack as \attack.
% Additionally, there are two other attacks which could also construct the deterministic path, named \latent and \context (more details are shown in the appendix). However, they address the stochastic problem by attacking only the deterministic components, i.e., encoders, as opposed to our end-to-end attacks for the entire model. We corroborate this claim with empirical evaluations and include more details about these attacks in the Appendix. 

\textbf{Component 2: Additional Objective Functions for Outer Minimization.}
To better learn a robust trajectory prediction model,
we need to bound $|f(\mathbf{X}+\delta) - f(\mathbf{X})|$ so that the latent condition variable of the adversarial input is close to that of the unperturbed input. %To do so, we propose to regularize the conditional variable $\mathbf{C}$. 
We propose the following regularization loss $\mathcal{L}_\text{reg}$:
\begin{equation}
\label{eq:reg}
% \mathcal{L}_\text{reg} = \mathrm{d}(\,f(\mathbf{X},\mathbf{X} + \delta)\,)
\mathcal{L}_\text{reg} = \mathrm{d}( f(\mathbf{X}+\delta), f(\mathbf{X}))
\end{equation}
, where $\mathrm{d}$ is a distance function (i.e. we use $L_2$ norm as the distance metric).

In addition, because the clean data has a fixed distribution, simultaneously learning from the clean data during the adversarial training process anchors the conditional distribution on a stable clean data distribution.
Specifically, we leverage the following loss:
\begin{equation}
\label{eq:clean}
\mathcal{L}_\text{clean}(\mathbf{X}, \mathbf{Y}) = \mathcal{L}_\text{total}(\mathbf{X},\mathbf{Y}) 
\end{equation}
where $\mathcal{L}_\text{total}$ could be the loss in Eq.~\ref{eq:cvae_loss} for CVAE-based model or Eq.~\ref{eq:cgan_loss} for cGAN-based model.

\textbf{Component 3: Data Augmentation.}
To further improve the trade-offs between the performance on clean and adversarial data,
we need to address the overfitting problem of the min-max adversarial training~\cite{rice2020overfitting}. 
Data augmentation is shown to be effective in addressing the problem in the image classification domain~\cite{rebuffi2021fixing}. 
However, data augmentation in trajectory prediction is rarely studied and non-trivial. To design an effective augmentation algorithm, Rebuffi et al.~\cite{rebuffi2021fixing} argues that the most important criterion is that the augmented trajectories should also be realistic. 
Thus, we design a dynamic-model based data augmentation strategy $A$ shown in the appendix. By using the augmentation, we can generate diverse, realistic multi-agent trajectories for each scene and construct $\mathbb{D}_{aug}$. 
% More details for the dynamic-model-based augmentation will be discussed in the Appendix.



% Thus, we design a dynamic-model based data augmentation strategy $A$ as follows. 
% We use a kinematic bicycle model~\cite{MATUTE2019kinematic} as our dynamic model to generate realistic trajectories that can be driven in the real world. Representing the behavior of actors as kinematic bicycle model trajectories allows for physical feasibility and fine-grained behavior control. 
% To generate realistic trajectories, we first parameterize the trajectory $\mathbf{S}=\{s^t\}_0^T$ as a sequence of kinematic bicycle model states $s^t = \{p^t, \kappa^t, a^t\}$, where $p$ represents the position, $\kappa$ represents the trajectory curvature, and $a$ represents the acceleration. Then, trajectories can be generated by controlling the change of curvature $\Dot{\kappa}_t$ and the acceleration $a_t$ over time, and using the kinematic bicycle model to update corresponding other states for each timestamp. 
% To generate diverse trajectories, we set the objectives as biasing the trajectories to a given direction (e.g. forward, backward, left and right), while not colliding with other agents. To that end, we optimize a carefully-designed objective function $\mathcal{L}_\text{dyn}$ over the control actions, i.e. $\Dot{\kappa}_t$ and $a_t$ for each agents. More specifically, the objective function consists of two components:
% $\mathcal{L}_\text{dyn} = \mathcal{L}_\text{d} + \gamma \mathcal{L}_\text{col}$
% , where $\mathcal{L}_\text{d}$ is the deviation objective loss, $\mathcal{L}_\text{col}$ is the collision regularization loss, and $\gamma$ is a weight factor to balance the objectives. In each scene, we randomly pick a deviation objective loss $\mathcal{L}_\text{d}$ from the set ($\{$moving forward, backward, left, right$\}$ for each agent. We also clip the maximum deviation of the positions so that the trajectories are constrained to be in the lane. 
% By doing so, we can generate diverse, realistic multi-agent trajectories for each scene and construct $\mathbb{D}_{aug}$. More details for the dynamic-model-based augmentation will be discussed in the Appendix.


To summarize, our adversarial training strategy for trajectory prediction models could be formulated as follows:
\begin{equation}\label{eq:robust_traj}
\vspace{-0.2em}
\begin{split}
     \delta =& \argmax_{\delta \in \mathbb{S}} \mathcal{L}_\text{adv}(\,\mathbf{X} + \delta,  \mathbf{Y}), \quad\text{where}  \{\mathbf{X},\mathbf{Y}\} \in \mathbb{D} \cup \mathbb{D}_{aug}\\
     \theta,\,\phi  =& \argmin_{ \theta,\,\phi} \mathcal{L}_\text{total}(\mathbf{X}+\delta,\mathbf{Y}) + \mathcal{L}_\text{clean}(\mathbf{X},\mathbf{Y}) + \beta\cdot \mathcal{L}_\text{reg}(\, \mathbf{X},\, \mathbf{X}+\delta\,)
\end{split}
\end{equation}
% \begin{equation}
% \label{eq:robust_traj}
% % $
% %     \{\mathbf{X},\mathbf{Y}\} \in \mathbb{D} \cup \mathbb{D}_{aug} \quad
% %      \delta = \argmax_{\delta \in \mathbb{S}} \mathcal{L}_\text{adv}(\,\mathbf{X} + \delta,  Y);\, \theta,\,\phi  =  \mathcal{L}_\text{total}(\mathbf{X}+\delta,\mathbf{Y}) + \mathcal{L}_\text{clean}(\mathbf{X},\mathbf{Y}) + \beta\cdot \mathcal{L}_\text{reg}(\, \mathbf{X},\, \mathbf{X}+\delta\,)
% % $
% \begin{split}
%     & \{\mathbf{X},\mathbf{Y}\} \in \mathbb{D} \cup \mathbb{D}_{aug} \\
%      \delta =& \argmax_{\delta \in \mathbb{S}} \mathcal{L}_\text{adv}(\,\mathbf{X} + \delta,  Y)\\
%      \theta,\,\phi  =& \mathcal{L}_\text{total}(\mathbf{X}+\delta,\mathbf{Y}) + \mathcal{L}_\text{clean}(\mathbf{X},\mathbf{Y}) + \beta\cdot \mathcal{L}_\text{reg}(\, \mathbf{X},\, \mathbf{X}+\delta\,)
% \end{split}
% \end{equation}
, where $\mathbb{D}$, $\mathbb{D}_\text{aug}$ are the training data and augmented data; $\mathcal{L}_\text{adv}$ is  adversarial loss  to generate effective adversarial examples in Eq.~\ref{eq:adv_loss}; $\mathcal{L}_\text{total}$ is the loss in Eq.~\ref{eq:cvae_loss} and Eq.~\ref{eq:cgan_loss} to train a robust model against adversarial examples generated from Eq.~\ref{eq:adv_loss}; $\mathcal{L}_\text{reg}$ and $\mathcal{L}_\text{clean}$ are loss shown in Eq.~\ref{eq:reg}  and Eq.~\ref{eq:clean} to provide a stable signal for training.  $\beta$ is a hyperparameter for adjusting the regularization.
